Continuous Curve Textures

Repetitive patterns are ubiquitous in natural and human-made objects, and can be created with a variety of tools and methods. Manual authoring provides unmatched degree of freedom and control, but can require significant artistic expertise and manual labor. Computational methods can automate parts of the manual creation process, but are mainly tailored for discrete pixels or elements instead of more general continuous structures. We propose an example-based method to synthesize continuous curve patterns from exemplars. Our main idea is to extend prior sample-based discrete element synthesis methods to consider not only sample positions (geometry) but also their connections (topology). Since continuous structures can exhibit higher complexity than discrete elements, we also propose robust, hierarchical synthesis to enhance output quality. Our algorithm can generate a variety of continuous curve patterns fully automatically. For further quality improvement and customization, we also present an autocomplete user interface to facilitate interactive creation and iterative editing. We evaluate our methods and interface via different patterns, ablation studies, and comparisons with alternative methods.

==> assisting_operator.tex <==
\section{Assisting Operator}
\label{sec:AssistingOperator}

\textit{Assisting operators} generate auxiliaries distributed across space. Inspired by partition operator proposed by \cite{Loi:2017:PAE}, our system support regular and non-regular assistance. We also support constrained assistance by allowing the users to provide control maps.
The assisting operator is applied to enclosed regions $R$ and generates auxiliaries that forms enclosed subregions. It might not be necessary to form enclosed subregions, however, it makes our operator concise and easy to define.

\subsection{Basic assistance}
\label{subsec:BasicAssistance}

We support stripe, grid \cite{Loi:2017:PAE}, cake-like \cite{Tu:2018:CLP}, uniform, random assisting operators that generate auxiliary lines and points.

\begin{equation*}
stripeAssistance(\phi,d): R \rightarrow \{\auxiliary\}
\end{equation*}
where $\phi$ represents the angle of stripes. $d$ represents the distance between neighboring stripes. 
\begin{equation*}
	gridAssistance(\phi_1,\phi_2,d_1,d_2,h): R \rightarrow \{\auxiliary\}
\end{equation*}
where $\theta_1$, $\theta_2$ represent the angles of two stripes respectively. $d_1$, $d_2$ represent the distances.
\begin{equation*}
	cakeAssistance(n,h): R \rightarrow \{\auxiliary\}
\end{equation*}
\begin{equation*}
	uniformAssistance(n,h): R \rightarrow \{\auxiliary\}
\end{equation*}
\begin{equation*}
	randomAssistance(n,h): R \rightarrow \{\auxiliary\}
\end{equation*}
where $n$ represents the number of auxiliary lines to be generated within $R$. $h$ indicates the mode of auxiliaries generations, for example, generating only auxiliary lines, only points or both. Please refer to the supplement for more details. 

\subsection{Constrained assistance}
\label{subsec:ConsPartition}
Users can provide additional control maps to constrain the auxiliary generation. 
\begin{equation*}
	constrainedAssistance(\{C\},h): R
\end{equation*}
where $\{C\}$ represents control maps indicating element orientation, size or density etc. The algorithm is based on anisotropic and multi-class blue noise sampling \cite{Li:2010:ABN} and \cite{Wei:2010:MBN}.
  


\nothing{

\subsection{Example-based assistance}
Users might want to easily produce some complex partitions without involving too much effort on procedure design.
Example-based partition allows users to design their own partition within a small space, and our system will automatically synthesize more auxiliaries within a large space using \cite{Oztireli:2012:ASP,Ma:2011:DET}.
But it should be noted that this function can only provide limited quality on large structural partitions.

\begin{equation*}
exampleBasedAssistance(\{obj^1\}): R
\end{equation*}

}



==> dart_throw_alg.tex <==
\begin{algorithm}
  \begin{algorithmic}[1]
  	
   \REQUIRE sample domain $\domainsym$ with distance $\dist$ and conflict $\conflictdist$ measure
    \ENSURE output sample set $\sampleset$
    \STATE $\sampleset \assign \emptyset$
    \STATE $\failure \assign 0$ \pcomment{failure count}
    \WHILE{$\domainsym$ is not fully covered and $\failure$ not too high}
    \STATE $\sample \assign \funct{RandomSample}(\domainsym)$
    \IF{$\dist(\sample, \sampleprime) < \conflictdist(\sample, \sampleprime) \; \forall \sampleprime \in \sampleset$}
    \STATE $\sampleset \assign \sampleset \union \sample$ \pcomment{accept trial sample}
    \STATE $\failure \assign 0$
    \ELSE
    \STATE $\failure \assign \failure + 1$
    \ENDIF
    \ENDWHILE
    \RETURN{} $\sampleset$
  \end{algorithmic}
  \Caption{Dart throwing.}
  {%
This is an example of pseudo-code.
  }
  \label{alg:dart_throw}
\end{algorithm}




==> fig_ablation_curve_recon.tex <==
\begin{figure}[ht]

\nothing{
	\subfloat[exemplar]{
	\label{fig:curve_recon:exemplar:1}
	\includegraphics[width=0.22\linewidth]{figs/method/ablation/exemplar_crocodile_skin.jpg}
}%
	\subfloat[without  orientation attribute]{
	\label{fig:curve_recon:without:1}
	\includegraphics[width=0.38\linewidth]{figs/method/curve_recon/graph.pdf}
}%
	\subfloat[with orientation attribute]{
	\label{fig:curve_recon:with:1}
	\includegraphics[width=0.38\linewidth]{figs/method/curve_recon/graph.pdf}
}%

	\subfloat[exemplar]{
	\label{fig:curve_recon:exemplar:2}
	\includegraphics[width=0.22\linewidth]{figs/results/more_results/exemplar_flame.jpg}
}%
\subfloat[without  orientation attribute:2]{
	\label{fig:curve_recon:without:2}
	\includegraphics[width=0.38\linewidth]{figs/method/curve_recon/graph.pdf}
}%
\subfloat[with orientation attribute:2]{
	\label{fig:curve_recon:with}
	\includegraphics[width=0.38\linewidth]{figs/method/curve_recon/graph.pdf}
}%

	\Caption{Reconstruction with or without orientation attributes}
{%
%
}
\label{fig:ablation:curve_recon}

}%
\end{figure}


==> fig_edge_assignment.tex <==
\begin{figure}[H]
  \centering
  \subfloat[initial graph reconstruction]{
    \includegraphics[width=0.33\linewidth]{figs/results/continuous_synthesis/recon_graph_example_random_rectangles_continuous_n0_80_n1_60_n2_40.jpg}
  }%
  \subfloat[graph denoising (previous)]{
  	\label{fig:graph_denoising:1}	\includegraphics[width=0.333\linewidth]{figs/results/continuous_synthesis/denoised_graph_example_random_rectangles_continuous_n0_80_n1_60_n2_40}
}%
  \subfloat[optimization (now)]{
  	  	\label{fig:optimization:1}
    \includegraphics[width=0.333\linewidth]{figs/results/continuous_synthesis/edge_assignment_graph_example_random_rectangles_continuous_n0_80_n1_60_n2_40}
  }%

  \subfloat[initial graph reconstruction]{
	\includegraphics[width=0.333\linewidth]{figs/results/continuous_synthesis/recon_graph_example_circles_continuous_n0_80_n1_60_n2_40.jpg}
	}%
	\subfloat[graph denoising (previous)]{
		  	\label{fig:graph_denoising:2}
		\includegraphics[width=0.333\linewidth]{figs/results/continuous_synthesis/denoised_graph_example_circles_continuous_n0_80_n1_60_n2_40.jpg}
	}%
	\subfloat[optimization (now)]{
	      \label{fig:optimization:2}
		\includegraphics[width=0.33\linewidth]{figs/results/continuous_synthesis/edge_assignment_graph_example_circles_continuous_n0_80_n1_60_n2_40}
	}%

 \Caption{Graph reconstruction.}
 {%
 	The edge assignment (optimization) and graph denoising produces very similar results. 
 	Sometimes edge assignment \subref{fig:optimization:1} is better (also, the optimization is non-convex. We don't produce the same results every time. I am using an open-source optimization software. There should be some random number generator inside the software implementation), and sometimes denoising \subref{fig:graph_denoising:2} produces better results.
 	We may not have much to investigate regarding this step.
 }
 \label{fig:edge_assignment}
\end{figure}


==> fig_edge_assignment_issue.tex <==
\begin{figure}[htb]
  \centering
    \includegraphics[width=\linewidth]{figs/method/edge_assignment_issue.pdf}

 \Caption{A potential edge assignment issue.}
 {
	If we compute each edge separately, we are unlikely avoid to generate such small unpleasing cycles (orange edges).
 }
 \label{fig:edge_assignment_issue}
\end{figure}


==> fig_init_robust_synthesis.tex <==
\begin{figure}[htb]
  \centering
  \subfloat[exemplar]{
    \label{fig:robust_synthesis_exemplar}
    \includegraphics[width=0.5\linewidth]{figs/method/init_robust_synthesis_exemplar.png}
  }%
  \subfloat[unrobust synthesis (previous result)]{
	\label{fig:unrobust_synthesis_result}
	\includegraphics[width=0.5\linewidth]{figs/method/unrobust_synthesis_result.jpg}
}%

  \subfloat[robust synthesis]{
    \label{fig:robust_synthesis_result}
    \includegraphics[width=0.8\linewidth]{figs/method/init_robust_synthesis_result.png}
  }%

 \Caption{An initial robust synthesis result.}
 {%
		\subref{fig:robust_synthesis_result} is generated by robust matching (\Cref{sec:neighborhood_matching:robust}) with adaptive sampling (\Cref{subsubsec:adaptive_sampling}). 
 }
 \label{fig:robust_synthesis}
\end{figure}


==> fig_initial_recon_results.tex <==
\begin{figure}[htb]
  \centering
    \includegraphics[width=\linewidth]{figs/method/InitReconstruction.png}

 \Caption{Initial reconstruction results}
 {
 	The red points are samples. The green line indicates reconstructed edges.
 %
 }
 \label{fig:init_recon_results}
\end{figure}


==> fig_initial_results.tex <==
\begin{figure}[htb]
  \centering
    \includegraphics[width=\linewidth]{figs/method/InitSynthesisResult.png}

 \Caption{Initial results}
 {%
 The short directional edges represent the orientations of potential edges. 
 The colors (green and blue, except red) of the sample node represents the potential number of edges associated with the node. Red are example samples.
 In this screenshot, green represents two and blue three. The yellow path indicates user-specified autocomplete domain. 
 }
 \label{fig:init_results}
\end{figure}


==> fig_realistic_results.tex <==
\begin{figure*}[htb]
  \centering
  \subfloat[regular brick wall]{
    \includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/bricks.jpg}
  }%
  \subfloat[synthesized]{
    \label{fig:realistic_results:brick:synthesized}
    \includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_bricks_n0_80_n1_60_n2_30.jpg}
  }%
  \subfloat[irregular brick wall]{
  	\label{fig:realistic_results:irregular_brick_wall:example}
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/random_bricks.jpg}
}%
\subfloat[synthesized]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_random_bricks_n0_80_n1_60_n2_40.jpg}
}%
  \subfloat[crocodile skin]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/crocodile_skin.jpg}
}%
\subfloat[synthesized]{
		\label{fig:realistic_results:crocodile_skin:synthesized}
	\includegraphics[width=0.07\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_crocodile_skin_n0_80_n1_60_n2_40_old.jpg}
	\includegraphics[width=0.07\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_crocodile_skin_n0_70_n1_55_n2_40_new.jpg}
}%
  \subfloat[branches]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/tree.jpg}
}%
\subfloat[synthesized]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_tree_n0_80_n1_60_n2_40.jpg}
}%

  \subfloat[wave]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/random_curves.jpg}
}%
\subfloat[synthesized]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_random_curves_n0_80_n1_60_n2_40.jpg}
}%
  \subfloat[maze]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/mostof.jpg}
}%
\subfloat[synthesized]{
    \label{fig:realistic_results:maze:synthesized}
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_mostof_n0_60_n1_50_n2_40}
}%
  \subfloat[cell]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/very_random_cell.jpg}
}%
\subfloat[synthesized]{
	 \label{fig:realistic_results:cell:synthesized}
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_very_random_cell_n0_80_n1_60_n2_40}
}%
  \subfloat[Distorted grids]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curvy_grids.jpg}
}%
\subfloat[synthesized]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_curvy_grids_n0_80_n1_60_n2_30}
}%

  \subfloat[Leaves]{
  	\label{fig:realistic_results:leaves}
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/leave_big.jpg}
}%
\subfloat[synthesized]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_leave_big_demo_n0_60_n1_50_n2_40}
}%
  \subfloat[vertical lines]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/vertical.jpg}
}%
\subfloat[synthesized]{
    \label{fig:realistic_results:vertical:synthesized}
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_vertical_n0_80_n1_60_n2_40}
}
 \subfloat[Tree]{
		\label{fig:realistic_results:Tree}
		\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/exemplar_mixed_tree.jpg}
	}%
\subfloat[synthesized]{
		\label{fig:realistic_results:tree:synthesized}
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_mixed_tree_n0_70_n1_55_n2_40}
}%
 \subfloat[Grids]{
	\label{fig:realistic_results:grids}
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/exemplar_mixed_grids.jpg}
}%
\subfloat[synthesized]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_continuous_synthesis/curve_recon_mixed_grids_n0_70_n1_55_n2_40}
}%

 \subfloat[discrete leaves]{
	\label{fig:realistic_results:discrete_leaves}
	\includegraphics[width=0.12\linewidth]{figs/results/robust_discrete_synthesis/exemplar_example_leaves.jpg}
}%
\subfloat[synthesized]{
	\includegraphics[width=0.12\linewidth]{figs/results/robust_discrete_synthesis/curve_recon_example_leaves_n0_70_n1_55_n2_40}
}%



 \Caption{Realistic results.}
 {%
 	We are able to synthesize uniform or stochastic patterns without obvious artifacts fully automatically. For more structured patterns (such as \subref{fig:realistic_results:leaves}), human is easy to perceive artifacts .
 	I hope it's OK in the context of autocomplete systems.
 	Hierarchical pattern is possible with user interactions.
 	Note all patterns are reconstructed with B\'{e}zier curves. Sometimes it's better to reconstruct with polyline. There are artifacts on the boundary.
 }
 \label{fig:realistic_results}
\end{figure*}


==> fig_very_hierarchical_pattern.tex <==
\begin{figure}[htb]
	\centering
			\includegraphics[width=0.8\linewidth]{figs/examples/very_hierarchical_pattern.pdf}

	\Caption{Very hierarchical pattern}
	{%
		This pattern not only have global but local structures. I think it is necessary to synthesize such patterns by further sparsifying the representation: use a single sample to represent multiple elements. If we like, we can create such kind of very hierarchical patterns as many as possible. This can be very hard (according to my experience, it might be impossible) to synthesize by non-hierarchical method.

	}
	\label{fig:very_hierarchical_pattern}
\end{figure}


==> hierarchical_pattern_fig.tex <==
\begin{figure}[tbh!p]
\centering
\includegraphics[width=\linewidth]{figs/categories/hierarchical_pattern.jpg}
\Caption{Hierarchical pattern example.}
{There are identifiable repetitive elements in this pattern. The largest element is a branch. Besides shape transformations, the branches have substantial variations (e.g. more or less sub-branches, leaves).
The sub-branch and leaf are sub-elements that also exhibit repetitions.
}
\label{fig:hierarchical_pattern}
\end{figure}


==> hierarchical_sampling_fig.tex <==
\begin{figure}[tbh!p]
  \centering
  \includegraphics[width=\linewidth]{figs/categories/crop_complex_texture_ec_1_samples.pdf}
  \Caption{Hierarchical sampling example.}
  {
The synthesis can progress for coarse to fine level samples (e.g. red first, then green, and finally magenta), or weigh them differently with different neighborhoods (e.g. larger neighborhoods and heavier weights for coarser-level samples).
%
  }
  \label{fig:hierarchical_sampling}
\end{figure}


==> other_operator.tex <==
\section{Other Functional Operator}
\subsection{Retag operator}
\textit{Retag operator} can alter the type or group of $obj$.
\subsection{Merging Operator}
Similar to \cite{Loi:2017:PAE}.

\subsection{Object Selector and Deleter}
The users can easily select objects they want to edit (e.g. retag). 



\subsection{Easy Parameter Setting}
The system has many user-defined parameters.
However, if the parameters are unnaturally fixed, the resulting pattern might look unpleasing. We provide functions to assist the users setting parameters.

\subsubsection{Continuous parameters}

\begin{equation*}
randomC(a,b):\{{p}\}
\end{equation*}
\begin{equation*}
linspace(a,b):\{{p}\}
\end{equation*}
where $randomC$ produce uniform distribution ranging between [a,b], $linspace$ produce $n$ numbers equally spacing between [$a$,$b$]. $\{p\}$ are the parameters the users want to set. 

\subsubsection{Discrete parameters}

\begin{equation*}
	randomD(\{id^*\}):\{id\}
\end{equation*}
where $randomD$ randomly assign tag $id^*$ to $id$ with equal probability.

